Reconstruction guided Meta-learning for Few Shot Open Set Recognition

In many applications, we are constrained to learn classifiers from very limited data (few-shot classification). The task becomes even more challenging if it is also required to identify samples from unknown categories (open-set classification). Learning a good abstraction for a class with very few samples is extremely difficult, especially under open-set settings. As a result, open-set recognition has received minimal attention in the few-shot setting. However, it is a critical task in many applications like environmental monitoring, where the number of labeled examples for each class is limited. Existing few-shot open-set recognition (FSOSR) methods rely on thresholding schemes, with some considering uniform probability for open-class samples. However, this approach is often inaccurate, especially for fine-grained categorization, and makes them highly sensitive to the choice of a threshold. To address these concerns, we propose Reconstructing Exemplar-based Few-shot Open-set ClaSsifier (ReFOCS). By using a novel exemplar reconstruction-based meta-learning strategy ReFOCS streamlines FSOSR eliminating the need for a carefully tuned threshold by learning to be self-aware of the openness of a sample. The exemplars, act as class representatives and can be either provided in the training dataset or estimated in the feature domain. By testing on a wide variety of datasets, we show ReFOCS to outperform multiple state-of-the-art methods.

==> tables/table_lambdas.tex <==

\begin{table}[h]
\centering
\scalebox{0.8}{
\begin{tabular}{@{}lcccccccc@{}} 
\toprule
\textsc{Datasets }   & \multicolumn{2}{c}{GTSRB$\rightarrow$GTSRB } & \multicolumn{2}{c}{GTSRB$\rightarrow$TT100K } & Belga$\rightarrow$Flickr32  & Belga$\rightarrow$Toplogos  & \multicolumn{2}{c}{\textit{mini}ImageNet$\rightarrow$\textit{mini}ImageNet }  \\ 
\midrule
\textsc{Experiment}  & $5$-way $5$-shot  & $5$-way $1$-shot         & $5$-way $5$-shot  & $5$-way $1$-shot          & $5$-way $1$-shot            & $5$-way $1$-shot            & $5$-way $1$-shot  & $5$-way $1$-shot                                          \\ 
\midrule
$\lambda_1$ & \ \ \ \  $10^{-4}$ & \ \ \ \  $10^{-4}$             & \ \ \ \  $10^{-4}$      & \ \ \ \  $10^{-4}$              & \ \ \ \  $10^{-4}$                & \ \ \ \  $10^{-4}$                & \ \ \ \  $10^{-4}$    & \ \ \ \  $10^{-4}$                                              \\
$\lambda_2$ & 10   & 10                       & 10                & 10                        & 10                          & 10                          & 1                 & 1                                                         \\
$\lambda_3$ & 10                & 10                       & 5                 & 10                        & 10                          & 10                          & 10                & 10                                                        \\
\bottomrule
\end{tabular}
}
\caption{\textbf{Choice of Loss function hyperparameters for all the few-shot experiments.} }
\label{tab:lambdas}
\end{table}

==> tables/table_supp_abl_belga.tex <==
\begin{table}[ht]
\renewcommand{\arraystretch}{1.5}
% \scriptsize
\centering
\resizebox{0.7\textwidth}{!}{
\begin{tabular}{@{}lcccc@{}}
\toprule
                                & \multicolumn{2}{c}{\textsc{Belga}$\rightarrow$\textsc{Flickr32}} & \multicolumn{2}{c}{\textsc{Belga}$\rightarrow$\textsc{Toplogos}}                              \\ 
\textsc{Experiment}                      &  \multicolumn{2}{c}{$5$-way $1$-shot}  &  \multicolumn{2}{c}{$5$-way $1$-shot}                         \\ \midrule
                                & \multicolumn{1}{c}{\textsc{Acc.}(\%)} & \multicolumn{1}{c}{\textsc{AUROC}(\%)} & \multicolumn{1}{c}{\textsc{Acc.}(\%)} & \multicolumn{1}{c}{\textsc{AUROC}(\%)}  \\ \midrule
Recons. w/ AE & 63.13 $\pm$ 1.05             & 71.86 $\pm$ 0.86           & 36.40 $\pm$ 2.00             & 56.37 $\pm$ 1.95     \\
No modulation         & 63.26 $\pm$ 1.03             & 56.69 $\pm$ 0.97       & 41.75 $\pm$ 1.99             & 52.83 $\pm$ 1.93              \\
ProtoC$+$ND     &    61.64 $\pm$   1.03                         &       50.01 $\pm$ 0.99            &    41.60 $\pm$ 2.04                         &       50.52 $\pm$ 2.06     \\
No embedding     &    65.49 $\pm$ 1.00                         &       67.79 $\pm$ 0.91        &    41.45 $\pm$ 2.01                         &       53.52 $\pm$ 2.11                    \\
No clf     &    64.51 $\pm$ 1.01                         &       71.58 $\pm$ 0.87            &    38.60 $\pm$ 1.96                        &       56.62 $\pm$ 1.86               \\
ReFOCS (Ours)                           & \textbf{66.29 $\pm$ 1.02}    & \textbf{72.98 $\pm$ 0.83}    & \textbf{42.30 $\pm$ 2.15}    & \textbf{58.39 $\pm$ 1.97}    \\ 
% \midrule
% & \multicolumn{2}{c}{\textsc{Belga}$\rightarrow$\textsc{Toplogos}}                              \\ 
% \textsc{Experiment}                      &  \multicolumn{2}{c}{$5$-way $1$-shot}                         \\ \midrule
%                                 & \multicolumn{1}{c}{\textsc{Acc.}(\%)} & \multicolumn{1}{c}{\textsc{AUROC}(\%)}  \\ \midrule
% Recons. w/ AE & 36.40 $\pm$ 2.00             & 56.37 $\pm$ 1.95                   \\
% No modulation         & 41.75 $\pm$ 1.99             & 52.83 $\pm$ 1.93                \\
% ProtoC$+$ND     &    41.60 $\pm$ 2.04                         &       50.52 $\pm$ 2.06                     \\
% No embedding     &    41.45 $\pm$ 2.01                         &       53.52 $\pm$ 2.11                         \\
% No clf     &    38.60 $\pm$ 1.96                        &       56.62 $\pm$ 1.86                           \\
% ReFOCS (Ours)                           & \textbf{42.30 $\pm$ 2.15}    & \textbf{58.39 $\pm$ 1.97}       \\
\bottomrule
\end{tabular}
}
\caption{\textbf{Ablation studies on brand logo recognition.} Recons. w/ AE refers to swapping the VAE with an Autoencoder (AE); No Modulation denotes turning off embedding modulation; No embedding/clf denote the removal of embedding/softmax scores from the input of the novelty module. ProtoC$+$ND refers to when we donot use exemplars for the reconstruction and consequently, remove the reconstruction errors from the input of the novelty module.}

% \vskip -0.1in
\label{tab:ablation_belga_whole}
\end{table}

==> tables/table_supp_abl_gtsrb.tex <==
\begin{table}[ht]
\renewcommand{\arraystretch}{1.5}
% \scriptsize
\centering
\resizebox{0.7\textwidth}{!}{
\begin{tabular}{@{}lcccc@{}}
\toprule
                                & \multicolumn{4}{c}{\textsc{GTSRB}$\rightarrow$\textsc{GTSRB}}                              \\ 
\textsc{Experiment}                      & \multicolumn{2}{c}{$5$-way $5$-shot}                         & \multicolumn{2}{c}{$5$-way $1$-shot}                         \\ \midrule
                                & \multicolumn{1}{c}{\textsc{Acc.}(\%)} & \multicolumn{1}{c}{\textsc{AUROC}(\%)} & \multicolumn{1}{c}{\textsc{Acc.}(\%)} & \multicolumn{1}{c}{\textsc{AUROC}(\%)} \\ \midrule
Recons. w/ AE & 94.11 $\pm$ 0.37             & 94.61 $\pm$ 0.32              & 83.83 $\pm$ 0.79             & 91.81 $\pm$ 0.45              \\
No modulation         & 93.11 $\pm$ 0.45             & 88.67 $\pm$ 0.55              & 84.34 $\pm$ 0.75             & 91.04 $\pm$ 0.54              \\
ProtoC$+$ND     &    89.72 $\pm$ 0.56                         &       82.23 $\pm$ 0.79                     & 82.79 $\pm$ 0.78             & 77.56 $\pm$ 0.92              \\
No embedding     &    93.55 $\pm$ 0.41                         &       88.80 $\pm$ 0.61                     & 85.78 $\pm$ 0.72            & 88.62 $\pm$ 0.61              \\
No clf     &    94.09 $\pm$ 0.35                         &       94.03 $\pm$ 0.34                     & 84.62 $\pm$ 0.78             & 92.10 $\pm$ 0.43              \\
ReFOCS (Ours)                           & \textbf{94.17 $\pm$ 0.38}    & \textbf{94.83 $\pm$ 0.35}     & \textbf{86.21 $\pm$ 0.78}    & \textbf{93.02 $\pm$ 0.45}     \\ 
\midrule
& \multicolumn{4}{c}{\textsc{GTSRB}$\rightarrow$\textsc{TT100K}}                              \\ 
\textsc{Experiment}                      & \multicolumn{2}{c}{$5$-way $5$-shot}                         & \multicolumn{2}{c}{$5$-way $1$-shot}                         \\ \midrule
                                & \multicolumn{1}{c}{\textsc{Acc.}(\%)} & \multicolumn{1}{c}{\textsc{AUROC}(\%)} & \multicolumn{1}{c}{\textsc{Acc.}(\%)} & \multicolumn{1}{c}{\textsc{AUROC}(\%)} \\ \midrule
Recons. w/ AE & 81.33 $\pm$ 0.80             & 77.08 $\pm$ 0.79              & 68.59 $\pm$ 0.88             & 75.71 $\pm$ 0.71              \\
No modulation         & 80.94 $\pm$ 0.79             & 78.55 $\pm$ 0.65              & 69.84 $\pm$ 0.91             & 77.75 $\pm$ 0.54              \\
ProtoC$+$ND     &    76.92 $\pm$ 0.83                         &       72.50 $\pm$ 0.61                     & 68.59 $\pm$ 0.83             & 71.61 $\pm$ 0.76              \\
No embedding     &    83.03 $\pm$ 0.75                         &       74.33 $\pm$ 0.66                     & 70.77 $\pm$ 0.87             & 59.28 $\pm$ 0.79              \\
No clf     &    82.71 $\pm$ 0.74                         &       82.85 $\pm$ 0.56                     & 69.14 $\pm$ 0.94             & 74.63 $\pm$ 0.61              \\
ReFOCS (Ours)                           & \textbf{83.36 $\pm$ 0.76}    & \textbf{85.25 $\pm$ 0.56}     & \textbf{71.45 $\pm$ 0.87}    & \textbf{81.98 $\pm$ 0.59}   \\
\bottomrule
\end{tabular}
}
\caption{\textbf{Ablation studies on traffic sign recognition.} Recons. w/ AE refers to swapping the VAE with an Autoencoder (AE); No Modulation denotes turning off embedding modulation; No embedding/clf denote the removal of embedding/softmax scores from the input of the novelty module. ProtoC$+$ND refers to when we donot use exemplars for the reconstruction and consequently, remove the reconstruction errors from the input of the novelty module.}

% \vskip -0.1in
\label{tab:ablation_gtsrb_whole}
\end{table}

==> tables/tables_tmp_traffic.tex <==
\begin{table}[ht]
\centering
\small
\resizebox{0.1\textwidth}{!}{
\begin{tabular}{llllllll}
\toprule
\multicolumn{1}{c}{\multirow{3}{*}[-5pt]{\textsc{Model}}}
% \multirow{3}{*}[-5pt]{\textsc{Model}}
& \multirow{3}{*}[-5pt]{\textsc{Metric}} 
& \multicolumn{4}{c}{\textsc{Datasets}} \\
\multicolumn{1}{c}{}  & 
& \multicolumn{2}{c}{\textsc{GTSRB}$\rightarrow$\textsc{GTSRB}}
& \multicolumn{2}{c}{\textsc{GTSRB}$\rightarrow$\textsc{TT100K}}  
\\ \cmidrule(l){3-8} 
\multicolumn{1}{c}{}  &
& \multicolumn{1}{c}{\textsc{Acc. (\%)}} 
& \multicolumn{1}{c}{\textsc{AUROC(\%)}} 
& \multicolumn{1}{c}{\textsc{Acc. (\%)}} 
& \multicolumn{1}{c}{\textsc{AUROC (\%)}} 
\\ \midrule
\multicolumn{4}{r}{5-way 5-shot} \\ \midrule
\textsc{ProtoNet \cite{proto_net}}     
& Euclidean                        
& 91.79 $\pm$ 0.44                      
& 70.74 $\pm$ 0.79           
& 80.51 $\pm$ 0.78    
& 62.10 $\pm$ 0.76  \\  
\textsc{Proto$+$OM \cite{open_max}}  
& Euclidean              
&  91.92 $\pm$ 0.43     
&  86.67 $\pm$ 0.48  
&  64.40 $\pm$ 0.78     
&  68.80 $\pm$ 0.66             \\
\textsc{PEELER \cite{peeler}}  
& Mahalanobis              
& 93.87 $\pm$ 0.37    
& 90.99 $\pm$ 0.44 
& 79.04 $\pm$ 0.79    
& 73.25 $\pm$ 0.81             \\
\textsc{ReFOCS}(Ours)  
& Cosine         
& \textbf{94.17 $\pm$ 0.38}   
& \textbf{94.83 $\pm$ 0.35}  
& \textbf{83.36 $\pm$ 0.76} 
& \textbf{85.25 $\pm$ 0.56}    \\ \midrule
\multicolumn{6}{r}{5-way 1-shot} \\ \midrule
\textsc{ProtoNet \cite{proto_net}} 
& Euclidean              
& 82.31 $\pm$ 0.75   
& 61.52 $\pm$ 0.90 
& 69.82 $\pm$ 0.87  
& 56.02 $\pm$ 0.83\\
\textsc{Proto$+$OM \cite{open_max}}  
& Euclidean              
& 82.46 $\pm$ 0.70  
& 81.43 $\pm$ 0.65 
& 55.10 $\pm$ 0.80    
& 67.79 $\pm$ 0.66           \\
\textsc{PEELER \cite{peeler}}
& Mahalanobis           
& 82.86 $\pm$ 0.77   
& 79.56 $\pm$ 0.85  
& \textbf{73.47 $\pm$ 0.88}   
& 69.68 $\pm$ 0.88       \\
\textsc{ReFOCS} (Ours)       
& Cosine       
& \textbf{86.21 $\pm$ 0.78}  
& \textbf{93.02 $\pm$ 0.45}     
& 71.45 $\pm$ 0.87      
& \textbf{81.98 $\pm$ 0.59}   \\ 
\bottomrule
\end{tabular}
}
\caption{\textbf{5-way 5-shot and 5-way 1-shot results of traffic sign and natural image classification}. For both traffic sign datasets GTSRB$\rightarrow$GTSRB and GTSRB$\rightarrow$TT100K, $800$ test episodes were evaluated and the average performance is reported. For the natural images the performance is averaged over $600$ test episodes. PEELER \textsuperscript{\textdied} denotes the corresponding results reported in \cite{peeler} while PEELER, in the previous row, denotes the results obtained via the official implementation \textsuperscript{\ref{url}}. All results are reported with $95\%$ confidence levels.}
\label{tab:traffic}
\vskip -0.1in
\end{table}
